Constant Approximation for Individual Preference Stable Clustering

Individual preference (IP) stability, introduced by Ahmadi et al. (ICML 2022), is a natural clustering objective inspired by stability and fairness constraints. A clustering is $\alpha$-IP stable if the average distance of every data point to its own cluster is at most $\alpha$ times the average distance to any other cluster. Unfortunately, determining if a dataset admits a $1$-IP stable clustering is NP-Hard. Moreover, before this work, it was unknown if an $o(n)$-IP stable clustering always \emph{exists}, as the prior state of the art only guaranteed an $O(n)$-IP stable clustering. We close this gap in understanding and show that an $O(1)$-IP stable clustering always exists for general metrics, and we give an efficient algorithm which outputs such a clustering. We also introduce generalizations of IP stability beyond average distance and give efficient, near-optimal algorithms in the cases where we consider the maximum and minimum distances within and between clusters.

==> alg-temp.tex <==
\section{An $O(\log n)$-Approximation to IP-Clustering}
In this section, we prove our main result. We show that for any set $P=\{x_1,\dots,x_n\}$ of $n$ points that form a metric space $(P,d)$ and every $k\leq n$, there exists a $k$-clustering $\mathcal{C}=(C_1,\dots,C_k)$ of $P$   which is $O(\log n)$-approximate IP-stable  (\cref{def:approx-ip}). Moreover, such a clustering can be found in time $\widetilde{O}(n^2 T)$, where $T$ is an upper bound on the time it takes to compute the distance between two points of $M$. 

% \begin{definition}\label{def:c-stable}
% A clustering of $X$ is $c$-IP stable if for every $x \in X$, the average distance from $x$ to members of its own cluster is at most $c$ times the average distance from $x$ to members of any other cluster. A clustering is called a $k$-clustering if $X$ is partitioned into $k$ disjoint non-empty clusters. 
% \end{definition}
\paragraph{Algorithm}
Our algorithm uses a subroutine,~\Cref{alg:main-subroutine}, which takes as input $P$ and a radius $r\in \mathbb{R}$ and returns a $t$-clustering $\mathcal{D}=(D_1,\dots,D_t)$ of $P$ with the properties that (1) for any $1\leq i\leq t$, the maximum distance between any two points of $ D_i$ is $O(r)$, and (2) for any $x\in P$ and any $i$ such that $x\notin D_i$, the average distance from $x$ to points of $D_i$ is $\Omega(r/\log n)$. These two properties ensure that $\mathcal{D}$ is $O(\log n)$-IP stable. However, we have no control on the number of clusters $t$ that the algorithm produces. To remedy this, we first run a greedy $k$-center algorithm on $P$ to obtain a set of centers $\{c_1,\dots,c_k \}$ and let $r_0$ denote the maximum distance from a point of $P$ to the nearest center. We then run~\Cref{alg:main-subroutine} with input radius $r=cr_0$ for some small constant $c$. This gives a clustering $\mathcal{D}=(D_1,\dots,D_t)$ where $t\geq k$. Moreover, we show that if we assign each cluster of $\mathcal{D}$ to the nearest center in $\{c_1,\dots,c_k \}$ (in terms of the minimum distance from a point of the cluster to the center), we obtain a $k$-clustering $\mathcal{C}=(C_1,\dots,C_k)$ which is $O(\log n)$-IP stable. The combined algorithm is~\Cref{alg:main} below.

We now describe the details of~\Cref{alg:main-subroutine}. The algorithm takes as input $n$ points $x_1,\dots,x_n$ of a metric space $(M,d)$ and a radius $r$. It first initializes a set $Q=\emptyset$ and then iteratively adds points $x$ from $P$ to $Q$ that are of distance at least $5r$ from points already in $Q$ such that $|P\cap B(x,r)|$,   the number of points within radius $r$ of $x$, is maximized. This is line 7--8 of the algorithm. 
Whenever a point $q_i$ is added to $Q$, we let $r_i=r$ and then iteratively increase $r_i$ by an additive $r/\lg n$ until the number of points of $P$ lying in the ``shell'' $B(q_i,r_i)\setminus B\left(q_i,r_i-\frac{r}{\lg n}\right)$ is at most half of the number of points of $P$ within $B(q_i,r_i)$. 
This is line 10--11 of the algorithm. 
The point of this process is to ensure that at least half the points of $P\cap B(q_i,r_i)$ are not too close to points outside $B(q_i,r_i)$. 
Note that each increase of $r_i$ (except for the last one) at least doubles the number of points in $P\cap B(q_i,r_i)$, and so $r_i$ can be increased at most $\lg n$ times which in turn implies that the final value of $r_i$ is at most $2r$. In particular, the balls $B(q_i,r_i)$ do not intersect. Finally, we create a cluster $D_i=B(q_i,r_i)$ for each $q_i\in Q$. This is line 13 of the algorithm. 
For any point $x\in P\setminus \bigcup_i D_i$, we find the minimum $i$ such that $d(x,q_i)\leq 6r$ and assign $x$ to $D_i$. 
This is line 16--18 of the algorithm. 
We finally return the clustering $\mathcal{D} =(D_1,\dots, D_t)$.


\begin{algorithm}[H]
\caption{\label{alg:main-subroutine} Clustering for a fixed radius}
\begin{algorithmic}[1]
\State \textbf{Input}: A set $P=\{x_1,\dots,x_n\}$ of $n$ points with a metric  $d$ and a radius $r>0$. 
\State \textbf{Output}: Clustering $\mathcal{D}=(D_1,\dots,D_t)$ of the points of $P$.
\Procedure{Ball-Carving}{$P,r$}
\State $Q\la \emptyset$
\State $i\la 1$
\While{there exists $x\in P$ with $d(x,Q)> 5r$}
\State $q_i\la$ a point $x\in P$ with $d(x,Q)> 5r$ maximizing $|P\cap B(x,r)|$
\State $Q\la Q\cup \{q_i\}$
\State $r_i \la r$
\While{$\left|B\left(q_i,r_i-\frac{r}{\lg n}\right)\cap P\right|< 2|B(q_i,r_i)\cap P| $ }
\State $r_i\la r_i+\frac{r}{\lg n}$
\EndWhile
\State $D_i\la B(q_i,r_i)$
\State $i\la i+1$
\EndWhile
\For{$x\in P$ assigned to no $D_i$}
\State $j\la\min\{i \mid d(x,q_i)\leq 6r\}$
\State $D_j\la D_j\cup \{x\}$
\EndFor
\State $t\la |Q|$
\State {\bf Return}: $\mathcal D = (D_1,\dots,D_t)$ 
\EndProcedure
\end{algorithmic}
\end{algorithm}

We next describe the details of~\Cref{alg:main}. The algorithm iteratively pick $k$ centers $c_1,\dots, c_k$ from $P$ for each center maximizing the minimum distance to previously chosen centers. For each center $c_i$, it initializes a cluster, starting with $C_i=\{c_i\}$. This is line 5--9 of the algorithm. Letting $r_0$ be the minimum distance between pairs of distinct centers, the algorithm runs~\Cref{alg:main-subroutine} on $P$ with input radius $r=r_0/11$ (line 10--11). This produces a clustering $\mathcal{D}$. In the final step, we iterate over the clusters $D$ of $\mathcal{D}$, assigning $D$ to the $C_i$ for which $d(c_i,D)$ is minimized (line 12--15). We finally return the clustering $(C_1,\dots,C_k)$. Our main result is as follows. 


\begin{algorithm}[H]
\caption{\label{alg:main} $O(\log n)$-approximate IP-clustering}
\begin{algorithmic}[1]
\State \textbf{Input}: Set $P=\{x_1,\dots,x_n\}$ of $n$ points with a metric  $d$ and integer $k$ with $2\leq k\leq n$. 
\State \textbf{Output}:  $k$-clustering $\mathcal{C}=(C_1,\dots,C_k)$ of the points of $P$.
\Procedure{IP-Clustering}{$P,k$}
\State $S\la \emptyset$
\For{$i=1,\dots,k$}
\State $c_i\la \argmax_{x\in P}\{d(x,S)\}$
\State $S\la S\cup\{c_i\}$
\State $C_i\la\{c_i\}$
\EndFor
\State $r_0\la \min\{d(c_i,c_j)\mid 1\leq i<j\leq k\}$
\State $\mathcal{D}\la$ \textsc{Ball-Carving}$(P,r_0/13)$\Comment{Call \cref{alg:main-subroutine}}
\For {$D\in \mathcal{D}$}
\State $j\la \argmin_i\{d(c_i,D)\}$ 
\State $C_j\la C_j\cup D$
\EndFor
\State {\bf Return}: $\mathcal{C} =(C_1,\dots,C_k)$ 
\EndProcedure
\end{algorithmic}
\end{algorithm}

\paragraph{Analysis} We now analyze our algorithm and provide its main guarantees.
\begin{theorem}\label{thm:main}
\cref{alg:main} outputs an $O(\log n)$-IP stable clustering in $O(n^2T + n^2 \log n)$ time.
\end{theorem}
In order to prove this theorem, we require the following lemma on~\Cref{alg:main-subroutine}.
\begin{lemma}\label{lem:main}
Let $(D_1,\dots,D_t)$ be the clustering output by~\Cref{alg:main-subroutine}. For each $i\in [t]$, the diameter of $D_i$ is at most $12r$. Further, for $x\in D_i$ and $j\neq i$, the average distance from $x$ to points of $D_j$ is at least $\frac{r}{3\lg n}$.
\end{lemma}
\begin{proof}
% For simplicity and without loss of generality, we assume that $M=P$. 
This gives a lighter notation as we will not have to take intersections with $P$ all the time. We may also assume that $n\geq 3$. We start out by noting that for each $i$, $r_i$ gets increased at most $\lg n$ times in line 10--11. To see this, suppose we increase $r_i$ $\ell\geq 1$ times. Initially, $B(q_i,r)$ must have contained at least $2$ points, namely $q_i$ and some point in $B(q_i,r)\setminus B(q_i,r-r/\lg n)$. Since, we increased $r_i$ $\ell$ times, the number of points in $B(q_i,r_i)$ must have doubled the first $\ell-1$ steps (otherwise, the condition in the while loop would not be satisfied). Therefore $2^{\ell}\leq n$, so $\ell\leq \lg n$. In particular the final value $r_i=r+\ell/\lg n\leq 2r$ and it follows by the triangle inequality that the balls $(B(q_i,r_i))_{i\in [t]}$ are disjoint. Moreover, after choosing the points in $Q$, it holds that $d(x,Q)\leq 5r$ for each $x\in P$ so the remaining unassigned points, do indeed get assigned to a cluster in line 16--18. This shows that $(D_1,\dots, D_t)$ is a partition of $P$ and moreover, that for each $i$, the diameter of $D_i$ is at most $12r$ (as each point in $D_i$ has distance at most $6r$ to $q_i$).

We proceed to prove the second statement of the theorem. Let $x\in D_i$ and $j\neq i$ be given and assume for contradiction that \[\frac{1}{|D_j|}\sum_{y\in D_j}d(x,y)< \frac{r}{3\lg n}.\] 
By Markov's inequality, \[\left|B\left(x,\frac{r}{\log n}\right)\cap D_j\right|> \frac{2}{3}|D_j|.\] Since $d(x,q_j)>r_j$, it holds by the triangle inequality that \[B\left(x,\frac{r}{\lg n}\right)\cap B\left(q_j,r_j-\frac{r}{\lg n}\right)=\emptyset\] and in particular, all points of $D_j\cap B\left(x,\frac{r}{\lg n}\right)$ must lie in the outer shell $B(q_j,r_j)\setminus B\left(q_j,r_j-\frac{r}{\lg n}\right)$. 
It follows that \[\left|B\left(q_j,r_j-\frac{r}{\lg n}\right)\right|<\frac{1}{3}|D_j|.\] By the condition of the while loop in line 10, it also holds that \[|B(q_j,r_j) \setminus B(q_j,r_j-\frac{r}{\lg n})|<\frac{1}{3}|D_j|\] and so, $|B(q_j,r_j)|<\frac{2}{3}|D_j|.$ 
In particular \[|B(q_j,r)|<|B(x,\frac{r}{\lg n})|\leq |B(x,r)|.\] 
However, when $q_j$ was added to $Q$ it was chosen as to maximize the number of points in $B(q_j,r)$ under the condition that $q_j$ had distance at least $5r$ to previously chosen points of $Q$. Since $|B(x,r)|> |B(q_j,r)|$, at the point $q_j$ was chosen, $Q$ already contained some point $q_{j_0}$ (with $j_0<j$) of distance at most $5r$ to $x$ and thus of distance at most $6r$ to any point of $|B(x,r-\frac{r}{\lg n})|$. 
Now since $|B(x,\frac{r}{\lg n})\cap D_j|> \frac{2}{3}|D_j|$, but the outer shell $B(q_j,r_j)\setminus B(q_j,r_j-\frac{r}{\lg n})$ contains at most $\frac{1}{3}|D_j|$ points of $D_j$, it must be the case that $B(x,\frac{r}{\lg n})$ contains more than $\frac{1}{3}|D_j|$ points of $D_j$ \emph{not in} $B(q_j,r_j)$. These points were assigned to $D_j$ in line 16--18 but this is a contradiction since $j_0<j_0$ and $q_{j_0}$ is also within distance $6r$ of each of them. This contradiction completes the proof.
\end{proof}
We are now ready to prove the the main result.
\begin{proof}[Proof of~\Cref{thm:main}]
Let us first argue about correctness.
% Again, we assume without loss of generality that $M=P$.
As each $c_i$ was chosen to maximize the minimal distance to points $c_j$ already in $S$, for any $x\in P$, it holds that $\min\{d(x,c_i)\mid i\in [k]\}\leq r_0$. 
By~\cref{lem:main}, in the clustering $\mathcal{D}$ output by \textsc{Ball-Carving}$(P,r_0/13)$ each cluster has diameter at most $\frac{12}{13}r_0<r_0$, and thus, for each $i\in [k]$, the cluster $D\in \mathcal{D}$ which contains $c_i$ will be included in $C_i$ in the final clustering. 
Indeed, in line 13 of~\cref{alg:main}, $d(c_i,D)=0$ whereas $d(c_j,D)\geq \frac{1}{13}r_0$ for all $j\neq i$. 
Thus, each cluster in $(C_1,\dots,C_k)$ is non-empty. Secondly, the diameter of each cluster is at most $4r_0$, namely, for each two points $x,x'\in C_i$, they are both within distance $r_0+\frac{12}{13}r_0<2r_0$ of $c_i$. 
Finally, by~\cref{lem:main}, for $x\in D_i$ and $j\neq i$, the average distance from $x$ to points of $D_j$ is at least $\frac{r_0}{39\lg n}$. 
Since, $\mathcal{C}$ is a coarsening of $\mathcal{D}$, i.e., each cluster of $\mathcal{C}$ is the disjoint union of some of the clusters in $\mathcal{D}$, it is straightforward to check that the same property holds for the clustering $\mathcal{C}$. 
 It follows that $\mathcal{C}$ is $O(\log n)$-approximate IP-stable.


We now analyze the running time. We claim that Algorithm \ref{alg:main} can be implemented to run in $O(n^2T + n^2 \log n)$ time, where $T$ is the time to compute the distance between any two points in the metric space. First, we can query all pairs to form the $n \times n$ distance matrix $A$. Then we sort $A$ along every row to form the matrix $A'$. Given $A$ and $A'$, we can easily implement our algorithms as follows. 

First, we argue about the greedy $k$-center steps of Algorithm $2$, namely, the for loop on line $5$. The most straightforward implementation computes the distance from every point to new chosen centers. At the end, we have computed at most $nk$ distances from points to centers which can be looked up in $A$ in time $O(nk) = O(n^2)$ as $k \le n$. In line $10$, we only look at every entry of $A$ at most once so the total time is also $O(n^2)$. The same reasoning also holds for the for loop on line $12$. It remains to analyze the runtime of Algorithm \ref{alg:main-subroutine}. 

Now given $r$, Algorithm \ref{alg:main-subroutine} can be implemented as follows. First, we calculate the size of $|B(x, r)|$ for every point $x$ in our dataset. This can easily be done by binary searching on the value of $r$ along each of the (sorted) rows of $A'$, which takes $O(n \log n)$ time in total. Similar to the $k$-center reasoning above, we can also pick the centers in Algorithm \ref{alg:main-subroutine} which are $> 5r$ apart iteratively by just calculating the distances from points to the chosen centers so far. This costs at most $O(n^2)$ time, since there are at most $n$ centers. 

Now suppose that we are growing the ball centered around a fixed point $x$ (the while loop on line $10$ of Algorithm \ref{alg:main-subroutine}). Consider the row in $A'$ corresponding to $x$. Suppose the ball currently has radius $r_i$ (which is initially equal to $r)$. We will maintain a pointer at the smallest entry in the row holding a distance larger than $r_i$ from $x$ as well as the count of $|B(x, r_i)|$ (initially $|B(x,r)|$ can be found via the binary step from before). If we are considering growing the the radius by $r/ \lg n$, we simply move the pointer from left to right until we encounter a distance larger than $r_i + r/\lg n$. While moving the pointer, we also keep track of the number of points which are at distance between $r_i$ and $r_i + r/\lg n$. Then we can simply compare this count with $|B(x,r_i)|$ and decide if we wish to keep growing the ball. If we do grow the ball, we can easily maintain the invariant that we know $|B(x,r_i)|$ as well. The key observation is that the pointer never moves to the left. Thus, in the worst case, the pointer only visits every entry of the row once, implying a $O(n)$ total runtime. Since there are at most $n$ balls that we grow, the total runtime of this step across all possible points $x$ is at most $O(n^2)$. This completes the runtime analysis.
\end{proof}
\begin{remark}
We note that the runtime can possibly be improved if we assume special structure about the metric space, such as a tree or Euclidean metric. In special cases, we can improve the running time by appealing to particular properties of the metric which allow us to either calculate distances or implement our subroutines faster. For example for tree metrics, all distances can be calculated in $O(n^2)$ time, even though $T = O(n)$. Likewise for the Euclidean case, we can utilize specialized algorithms for computing the all pairs distance matrix, which obtain speedups over the naive methods \cite{IndykSilwal2022}, or use geometric point location data structures to quickly compute quantities such as $|B(x,r)|$ \cite{Snoeyink04}. Our presentation is optimized for simplicity and generality so detailed discussions of specific metric spaces are beyond the scope of the work.
\end{remark}


\subsection{Tightness}

\begin{theorem}\label{thm:tight-bound}
For any $n$, there is a collection of $n$ points in $\R$ such that for any partition of the points into two nonempty sets $S_1, S_2$, there exist points $p, p'$ such that the average distance from $p$ to points in its set is at least $\Omega(\log n)$ times the average distance from $p'$ to points outside its set.
\end{theorem}
\begin{proof}
Let $\ell$ be the largest integer such that $n > 2^l - 1$.  Then place $1$ point at $0$, $2$ points at $1$ and so on until we place $2^{\ell-1}$ points at $\ell - 1$.  Finally place all of the remaining $n - 2^\ell + 1$ points at $l$.  Now one of the two sets $S_1, S_2$ in the partition must have at least $2^{\ell-2}$ points at $\ell - 1$, Without loss of generality, this is true for $S_1$.  Now consider the maximal (by value) point in $S_2$.  The average distance of this point to $S_1$ is $O(1)$.  Let this point be $p'$.  Now one of the two sets $S_1, S_2$ must have diameter at least $\lfloor \ell/2 \rfloor $ so in particular there is a point $p$ such that the average distance from $p$ to its set is at least $\Omega(\ell) = \Omega(\log n)$.  This proves the desired statement.   
\end{proof}

\section{Algorithm for Unweighted Trees}
In this section, we present an algorithm for IP-clustering on unweighted trees (where the distance $d(u,v)$ between two vertices $u$ and $v$ is number of edges on the unique path between them). As long as $k=O(n^{1/2}/\log n)$, it achieves an $O(1)$-approximate IP-clustering. The algorithm simply $k$-colors the vertices of the tree uniformly at random and groups together vertices of the same color in the same cluster. 
\begin{theorem}\label{thm:random-color}
Let $\gamma=O(1)$ and $k\leq c \frac{\sqrt{n}}{\log n}$ for a sufficiently small constant $c$. Let $T=(V,E)$ be an unweighted tree on $n$ nodes, and suppose that we $k$-color the vertices of $T$ randomly. Let $V_i$ denote the nodes of color $i$. With probability at least $1-n^{-\gamma}$, $(V_1,\dots, V_k)$ forms an $O(1)$-approximate IP-clustering.
\end{theorem}
We will first prove the following lemma. 

\begin{lemma}\label{lemma:random-color}
Let $\gamma=O(1)$ be a constant. There exists a constant $c>0$ (depending on $\gamma$) such that the following holds: Let $T=(V,E)$ be an unweighted tree on $n$ nodes rooted at vertex $r$. Suppose that we randomly $k$-color the nodes of $T$. Let $V_i\subseteq V$ be the nodes of color $i$, let $X_i=\sum_{v\in V_i}d(r,v)$, and let $X=\sum_{v\in V}d(r,v)$. If $k\leq c \frac{\sqrt{n}}{\log n}$, then with probability $1-O(n^{-\gamma})$, it holds that $X/2\leq kX_i\leq 2X$ for all $i\in[k]$.
\end{lemma}
\begin{proof}
%For $0\leq j< \lg M$, we denote by $W_j=\{v \in V: M/2^{j+1} < d(v,r)\leq M/2^j\}$. Note that $|W_j|\geq M/2^{j+1}-1$. Indeed, since the tree is unweighted, for every integer in $(M/2^{j+1},M/2^{j}]$, $W_j$ must contain a node of that distance to the root. 
We will fix $i$, and prove that the bound $X/2\leq X_i\leq 2X$ holds with probability $1-O(n^{-\gamma-1})$. Union bounding over all $i$ then gives the desired result. Let $\Delta=\max_{v\in V}d(r,v)$ be the maximum distance from the root to any vertex of the tree. We may assume that $\Delta\geq 5$ as otherwise the result follows directly from a simple Chernoff bound. Since the tree is unweighted and there exists a node $v$ of distance $\Delta$ to $r$, there must also exist nodes of distances $1,2,\dots,\Delta-1$ to $r$, namely the nodes on the path from $r$ to $v$. For the remaining nodes, we know that the distance is at least $1$. Therefore,
\[
\sum_{v\in V}d(r,v)\geq (n-\Delta-1 )+\sum_{j=1}^\Delta j=n+\binom{\Delta}{2}-1\geq n+\frac{\Delta^2}{3},
\]
and so $\mu_i=\E[X_i]\geq \frac{n+\Delta^2/3}{k}$. Since the variables $\left(d(r,v)[v\in V_i]\right)_{v\in V}$ sum to $X_i$ and are independent and bounded by $\Delta$, it follows by a Chernoff bound that for any $0\leq \delta\leq 1$,
\[
\Pr[|X_i-\mu_i|\geq \delta \mu_i]\leq 2\exp\left(-\frac{\delta^2\mu_i}{3\Delta} \right).
\]
By the AM-GM inequality, $\frac{\mu_i}{\Delta}\geq \frac{1}{k}\left(\frac{n}{\Delta}+\frac{\Delta}{3}\right)\geq \frac{2\sqrt{n}}{\sqrt{3}k}$. Putting $\delta=1/2$, the bound above thus becomes
\[
\Pr[|X_i-\mu_i|\geq  \mu_i/3]\leq 2\exp\left(-\frac{\sqrt{n}}{6\sqrt{3}k}\right)\leq 2\exp \left(-\frac{\sqrt{n}}{11k}\right)\leq 2n^{-\frac{1}{11c}},
\]
where the last bound uses the assumption on the magnitude of $k$ in the lemma. Choosing $c=\frac{1}{11(\gamma+1)}$, the desired result follows. 
\end{proof}


%Denote by $Z_{i,j}=\sum_{v\in V_i\cap W_j}d(r,v)=\sum_{v\in W_j}[v\in V_i]d(r,v)$ and $\mu_{i,j}=\E[Z_{i,j}]$. Note that 
%\[
%\mu_{i,j}=\frac{1}{k}\sum_{v\in W_j}d(r,v)\geq \frac{M}{k2^{j+1}}|W_j|%\geq \frac{M^2}{k2^{2j+3}}
%\]
%The variables $[v\in V_i]d(r,v)$ take values in the interval $[0,M/2^j]$, so it follows from a Chernoff bound that for $0\leq \delta \leq 1$,
%\[
%\Pr[|Z_{i,j}-\mu_{i,j}|\geq \delta \mu_{i,j}]
%\leq 2 \exp\left(-\delta^2 \frac{\mu_{i,j}}{3M/2^j}\right)\leq 2\exp\left(-\frac{\delta^2 |W_j|}{6k}\right).
%\]
%Choosing $\delta=1/2$, it follows that whenever $j$ is such that $|W_j|\geq \frac{(\gamma+2)k\log n}{24}$, then with probability $1-n^{-\gamma-2}$ that $\mu_{i,j}/2\leq Z_{i,j}\leq 3\mu_{i,j}/2$

\cref{thm:random-color} follows as a simple corollary:

\begin{proof}[Proof of~\cref{thm:random-color}]
Consider a node $u$ and let $X_i=\sum_{v\in V_i\setminus \{u\}}d(u,v)$. By~\cref{lemma:random-color}, the $X_i$'s are all within a constant factor of each other with probability $1-O(n^{-\gamma-1})$. Moreover, a simple Chernoff bound shows that with the same high probability \[|V_i|=\frac{n}{k}+O\left(\sqrt{\frac{n\log n}{k}}\right)=\Theta\left(\frac{n}{k}\right)\] for all $i\in [k]$. In particular, the values $Y_i=\frac{X_i}{| V_i\setminus \{u\}|}$ for $i\in[k]$ also all lie within a constant factor of each other which implies that $u$ is $O(1)$-stable in the clustering $(V_1,\dots,V_k)$. Union bounding over all nodes $u$, we find that with probability $1-O(n^{-\gamma})$, $(V_1,\dots,V_k)$ is an $O(1)$-approximate IP-clustering.
\end{proof}
\begin{remark}
The assumed upper bound on $k$ in Theorem~\ref{thm:random-color} is necessary (even in terms of the factor of $\log n$). Indeed, consider a tree $T$ which is a star $S$ on $n-k\log k$ vertices along with a path $P$ of length $k\log k$ having one endpoint at the center $v$ of the star. With probability $\Omega(1)$, some color does not appear on $P$. We refer to this color as color $1$. Now consider the color of the star center. With probability at least $9/10$, say, this color is different from $1$ and appears $\Omega(\log k)$ times on $P$ with average distance $\Omega(k\log k)$ to the star center $v$. Let the star center have color $2$. With high probability, each color appears $\Theta(n/k)$ times in $S$. Combining these bounds, we find that with constant probability, the average distance from $v$ to vertices of color $1$ is $O(1)$, whereas the average distance from $v$ to vertices of color $2$ is $\Omega\left(1+ \frac{k^2(\log k)^2}{n}\right)$.
In particular for the algorithm to give an $O(1)$-stable IP clustering, we need to assume that $k=O\left(\frac{\sqrt{n}}{\log n}\right)$.
\end{remark}

\section{Optimal Algorithm for Min-IP-Stable Clustering} 
We next consider the variant of the IP-clustering problem where, instead of looking at average distances, we aim to ensure that for any point $x$, the \emph{minimum} distance to a point in the cluster of $x$ is at most the minimum distance to a point in any other cluster. To be precise, for a set of points $P$ in a metric space $(M,d)$, we say that a clustering $\mathcal{C}=\{C_1,\dots,C_k\}$ is a \emph{min-IP-stable} $k$-clustering of $P$ if (1) $\mathcal{C}$ is a partition of $P$, (2) each $C\in \mathcal{C}$ is non-empty, and (3) for any $C\in \mathcal{C}$ such that $|C|\geq 2$ and any $x\in C$, it holds that $\min_{y\in C\setminus\{x\}}d(x,y)\leq \min_{y\in P\setminus C} d(x,y)$. 
We show that this version of the IP-clustering problem has an elegant solution, namely that a min-IP-stable $k$-clustering always exists for any value of $k\in [n]$ and moreover, can be found by a simple algorithm (\cref{alg:min-stab}) which we now describe.

The algorithm is identical to Kruskal's algorithm for finding a minimum spanning tree except that it stops as soon as it has constructed a forest with $k$ connected components. It first, initializes a graph $G=(V,E)$ with $V=P$ and $E=\emptyset$. Next, it computes all distances $d(x_i,x_j)$ between pairs of points $(x_i,x_j)$ of $P$ and sorts the pairs $(x_i,x_j)$ according to these distances. Finally, it goes through this sorted list adding each edge $(x_i,x_j)$ to $E$ if it connects different connected components of $G$. After computing the distances, it is well known that this algorithm can be made to run in time $O(n^2\log n)$, so the total running time is $O(n^2(T+\log n))$ where $T$ is the time to compute the distance between a single pair of points.
\begin{algorithm}[H]
\caption{\label{alg:min-stab} Exact min-IP-stable clustering}
\begin{algorithmic}[1]
\State \textbf{Input}: Set $P=\{x_1,\dots,x_n\}$ of $n$ points in a metric space $(M,d)$ and integer $k$ with $2\leq k\leq n$. 
\State \textbf{Output}: Min-stable $k$-clustering $\mathcal{C}=(C_1,\dots,C_k)$ of the points of $P$.
\Procedure{Min-IP-Clustering}{$P,k$}
\State $L\la \{(x_i,x_j)\mid 1\leq i <j \leq n\}$ sorted according to $d(x_i,x_j)$.
\State $E\la\emptyset$
\While{The graph $G=(P,E)$ has more than $k$ connected components}
\State $e\la$ an edge $e=(x,y)$ in $L$ with $d(x,y)$ minimal.
\State $L\la L\setminus\{e\}$
\If{$e$ connects different connected components of $G$}
\State $E\la E\cup\{e\}$
\EndIf
\EndWhile
\State $\mathcal{C}\la $ the connected components $(C_1,\dots,C_k)$ of $G$.
\State {\bf Return}: $\mathcal{C}$
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{theorem}\label{thm:min-IP-stable}
The $k$-clustering output by~\Cref{alg:min-stab} is a min-IP-stable clustering.
\end{theorem}
\begin{proof}
Let $\mathcal{C}$ be the clustering output by the algorithm. Conditions (1) and (2) in the definition of a min-stable clustering are trivially satisfied. To prove that (3) holds, let $C\in\mathcal{C}$ with $|C|\geq 2$ and $x\in C$. Let $y_0\neq x$ be a point in $C$ such that $(x,y_0)\in E$ (such an edge exists because $C$ is the connected component of $G$ containing $x$) and let $y_1$ be the closest point to $x$ in $P\setminus C$. When the algorithm added $(x,y_0)$ to $E$, $(x,y_1)$ was also a candidate choice of an edge between connected components of $G$. Since the algorithm chose the edge of minimal length with this property, $d(x,y_0)\leq d(x,y_1)$. Thus, we get the desired bound:
\[
\min_{y\in C\setminus\{x\}}d(x,y)\leq d(x,y_0)\leq d(x,y_1)= \min_{y\in P\setminus C} d(x,y). \qedhere
\]
\end{proof}

\section{\texorpdfstring{$3$}{3}-Approximation Algorithm for Max-IP-Stable Clustering}
We show that the well known greedy algorithm for the $k$-center problem results in a $3$-approximate max-IP-stable $k$-clustering.
\begin{theorem}\label{thm:max-IP-stable}
The $k$-clustering given by the standard greedy algorithm of $k$-center is $3$-approximate max-IP-stable.
\end{theorem}
\begin{proof}
To recall, the greedy algorithm of $k$-center (aka Gonzalez algorithm~\cite{gonzalez1985clustering}) starts with an arbitrary point as the first center and then goes through $k-1$ iterations. In each iteration, it picks a new point as a center which is furthest from all previously picked centers. Let $c_1, \cdots, c_k$ denote the selected centers and let $r := \max_{v\in P} d(v, \{c_1, \cdots, c_k\})$. Then, each point is assigned to the cluster of its closest center. We denote the constructed clusters as $C_1, \cdots, C_k$. Now, for every $i\neq j\in [k]$ and each point $v\in C_i$, we consider two cases:
\begin{itemize}
    \item{$d(v, c_i) \le r/2$.} 
        \begin{align*}
            \max_{u_i\in C_i} d(v,u_i) &\le d(v, c_i) + d(u_i, c_i) \le 3r/2, \\
            \max_{u_j\in C_j} d(v,u_j) &\ge d(v, c_j) \ge d(c_i, c_j) - d(v, c_i). \ge r/2
        \end{align*}    
    \item{$d(v, c_i) > r/2$.}
        \begin{align*}
            \max_{u_i\in C_i} d(v,u_i) &\le d(v, c_i) + d(u_i, c_i) \le 3d(v, c_i), \\
            \max_{u_j\in C_j} d(v,u_j) &\ge d(v, c_j) \ge d(v, c_i).
        \end{align*}
\end{itemize}
Hence, in both cases $\max_{u_i\in C_i} d(v,u_i) \le 3 \max_{u_j\in C_j} d(v, u_j)$.
\end{proof}
